A Knowledge Distillation Framework For Enhancing Ear-EEG Based Sleep Staging With Scalp-EEG Data

Sleep plays a crucial role in the well-being of human lives. Traditional sleep studies using Polysomnography are associated with discomfort and often lower sleep quality caused by the acquisition setup. Previous works have focused on developing less obtrusive methods to conduct high-quality sleep studies, and ear-EEG is among popular alternatives. However, the performance of sleep staging based on ear-EEG is still inferior to scalp-EEG based sleep staging. In order to address the performance gap between scalp-EEG and ear-EEG based sleep staging, we propose a cross-modal knowledge distillation strategy, which is a domain adaptation approach. Our experiments and analysis validate the effectiveness of the proposed approach with existing architectures, where it enhances the accuracy of the ear-EEG based sleep staging by 3.46% and Cohen's kappa coefficient by a margin of 0.038.

==> Sections/misc.tex <==
Humans spend one third of their lifetime in sleep, which is crucial to protect their mental and physical well-being. Sleep quality is difficult to assess  without compromising the comfort during the sleep of the patient, especially in clinical environment. Polysomnography (PSG), i.e sleep study, is a comprehensive and the gold standard test currently used to asses the quality of the sleep which supports the diagnosis of sleep disorders. PSG recordings consists of physiological signals such as Electroencephalogram (EEG), Electrocardiogram (ECG), Electromyogram (EMG), Electrooculogram (EOG) and SpO2 etc. 

During traditional sleep study, the patient will be wearing multiple sensors and electrodes. The quality of sleep is compromised due to the discomfort caused by these signal acquisition setup. Additionally, the setup is a complex, expensive and requires expert assistance thus prevents from being used in home-based sleep monitoring. Therefore, the sleep studies are conducted at sleep clinic, an unfamiliar environment to the patient, which will have a negative impact on the sleep quality, thus leads to errors in diagnosis.
 % and unfamiliarity of the clinical environment. 
 
In order to overcome the aforementioned challenges in sleep quality assessment, there have been several efforts to build a simple and comfortable system for high quality home-based sleep monitoring. Previous works have been focusing on utilizing either one or combinations of physiological signals such as Ear-EEG \cite{nakamura2019hearables, nakamura2017automatic, mikkelsen2017automatic, mikkelsen2019machine,tabar2021ear, mikkelsen2019accurate }, electrocardiogram (ECG) \cite{wei2019multi}, respiratory signal \cite{sun2019hierarchical}, electrooculogram (EOG) \cite{sun2019hierarchical}, heart rate (HR) \cite{zhang2018sleep}, photoplethysmography (PPG) \cite{korkalainen2020deep}, and actigraphy \cite{kapella2017actigraphy,zhang2018sleep} for sleep monitoring.



% One such method is to leverage ear-EEG \cite{kidmose_2013} for sleep monitoring. 
Ear-EEG is a potential alternative for scalp-EEG in sleep study, as
it contains similar information as scalp-EEG recordings in PSG \cite{kidmose_2013, mikkelsen2017keyhole}. Ear-EEG based sleep monitoring is advantageous because it provides comfort to the user compared to scalp-EEG and is portable which enables home-based sleep monitoring.   \cite{mikkelsen2017automatic,mikkelsen2019accurate} 
studied the possibilities of employing ear-EEG for automatic sleep staging by recording ear-EEG simultaneously with PSG of nine healthy subjects and employed a statistical classifier for sleep staging. The study strongly validated that the ear-EEG recordings contain necessary information on sleep stages and enable the classification of sleep stages with an acceptable level of accuracy. However, the performance on sleep staging using ear-EEG is significantly lower than scalp-EEG based sleep staging. This indicates that ear-EEG based sleep stage classification still has room for improvement in terms of accuracy and kappa scores. This accuracy gap could be due to the spatial difference in signal acquisition point and the signal-to-noise ratio discrepancy. %This indicates that the method in terms of accurate sleep staging is not quite on-par with the current gold-standard. 

We hypothesize that the sleep staging performance can be improved by utilizing deep-learning based techniques to transfer the knowledge from scalp-EEG to ear-EEG based classification methods. In order to achieve that we employ a well-known method named \emph{cross-domain knowledge distillation.} Here, a teacher model is initially trained on the scalp-EEG recordings in the manually annotated dataset. Then, the teacher model is fixed and we distill the knowledge to the student model by training it using ear-EEG recordings in a self-supervised manner. The experimental results validated our claim, which showed an improvement of $3.46\%$ in accuracy and $3.57\%$ in Cohen's kappa coefficient ($\kappa$).
%2.39, 1.8


% \begin{table*}[thpb] %thpb
% \caption{Results (USLEEP- Nature Paper 2021)}
% \label{tab:results}
% \begin{center}
% \scalebox{1}{
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\small{\bf Methods}} & \multirow{2}{*}{\small{\bf Metrics}} & \multirow{2}{*}{\small{\bf Subject 1}} & \multirow{2}{*}{\small{\bf Subject 2}} & \multirow{2}{*}{\small{\bf Subject 3}} & \multirow{2}{*}{\small{\bf Subject 4}} & \multirow{2}{*}{\small{\bf Subject 6}} & \multirow{2}{*}{\small{\bf Subject 7}} & \multirow{2}{*}{\small{\bf Subject 8}} & \multirow{2}{*}{\small{\bf Subject 9}} &
% \multirow{2}{*}{\small{\bf Average}} \\

% & & & & & & & & & &  \\
% \hline
% & & & & & & & & & &  \\
% scalp-EEG & \multirow{5}{*}{\small{Accuracy}} & 62.90 & 61.90 & 80.94 & 76.42 & 79.79 & 86.79 & 82.81 & 72.43 & \textbf{75.50} \\
% ear-EEG &  & 
% 32.89 & 64.52 & 71.15 & 70.26 & 79.81 & 83.75 & 74.69 & 57.50 & \textbf{66.82} \\

% TF & & 31.88 $\downarrow$ & 69.66 $\uparrow$ & 75.31 $\uparrow$ & 74.52 $\uparrow$ & 80.47 $\uparrow$ & 83.75 $\uparrow$ & 71.56 $\downarrow$ & 48.52 $\downarrow$ & \textbf{66.96 $\uparrow$}\\

% KD (Offline) & & 
% 32.80 \downarrow & 68.85 \uparrow & 71.56 \uparrow & 74.27 \uparrow & 80.14 \uparrow & 86.08 \uparrow & 73.00 \downarrow & 57.47 \downarrow & \textbf{68.02 $\uparrow$} \\
% KD (Online) & &  
% 36.14 \uparrow & 68.95 \uparrow & 75.83 \uparrow & 71.74 \uparrow & 80.34 \uparrow & 85.42 \uparrow & 80.00 \uparrow & 61.61 \uparrow & \textbf{70.00 $\uparrow$} \\
% & & & & & & & & & &  \\
% \hline
% & & & & & & & & & &  \\
% scalp-EEG & \multirow{5}{*}{\small{Kappa}} & 0.446 & 0.471 & 0.723 & 0.641 & 0.697 & 0.802 & 0.775 & 0.625 & \textbf{0.647} \\
% ear-EEG &  & 0.165 & 0.421 & 0.579 & 0.551 & 0.700 & 0.758 & 0.666 & 0.443 & \textbf{0.535} \\

% TF & & 0.159 $\downarrow$ & 0.503 $\uparrow$ & 0.644 $\uparrow$ & 0.604 $\uparrow$ & 0.703 $\uparrow$ & 0.754 $\downarrow$ & 0.630 $\downarrow$ & 0.331  $\downarrow$ & \textbf{0.541 $\uparrow$}\\


% KD (Offline) & & 0.148 $\downarrow$ & 0.455 $\uparrow$ & 0.607 $\uparrow$ & 0.589 $\uparrow$ & 0.698 $\downarrow$ & 0.795 $\uparrow$ & 0.638 $\downarrow$ & 0.446 $\uparrow$ & \textbf{0.547 $\uparrow$} \\

% KD (Online) & & 0.180 \uparrow & 0.507 \uparrow & 0.662 \uparrow & 0.572 \uparrow & 0.699 \downarrow & 0.784 \uparrow & 0.740 \uparrow & 0.487 \uparrow & \textbf{0.579 $\uparrow$}\\
% & & & & & & & & & &  \\
% \hline

% \end{tabular}}
% \end{center}
% \vspace{-2em}
% \end{table*}

==> tables/overall_results.tex <==
\begin{table*}[t]
% \begin{adjustwidth}{-2.25in}{0in} % Comment out/remove adjustwidth environment if table fits in text column.
\centering
\caption{{\bf Performance comparison between knowledge distillation, transfer learning and supervised learning for USleep \cite{usleep} and epoch cross-modal transformer\cite{pradeepkumar2022towards}}}

\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline  

\multirow{2}{*}{\textbf{ Model Architecture}}  & \multirow{2}{*}{\textbf{Modality}} &\multirow{2}{*}{\textbf{Method}}  & \multicolumn{6}{c}{\textbf{ {Overall Performance}}} \\ \cline{4-9}

 & & & {ACC} & $\kappa$ &  {MF1} &  {Sens.} &  {Spec.} &  {MGm}\\
\hline
 
 \multirow{5}{*}{USleep\cite{usleep}}   & Scalp EEG &  Supervised & 73.19  & 0.6313 & 61.51  & 64.12 & 92.8 & 77.13  \\
 \cline{2-9}
   & \multirow{4}{*}{Ear EEG} &  Supervised & 64.58 & 0.5236  & 56.04 & 58.11 & 90.84 & 72.66   \\
  & & TF    & 65.8 & 0.5331 & 55.73 & 57.42 & 90.96 & 72.27   \\
  & & KD (Offline)  &  66.25 & 0.5442 & 56.96 & 59.29 & 91.25 & 73.56  \\   
  & &  KD (Online)   & 68.04 & 0.5619 & 58.17 & 59.23 & 91.52 & 73.63  \\

  
 \hline

  & Scalp EEG &  Supervised & 77.76 & 0.6831 & 65.65 & 65.66 & 93.45 & 78.33  \\
 \cline{2-9}
   Epoch & \multirow{4}{*}{Ear-EEG} &  Supervised & 67.16 & 0.5378 & 56.25 & 56.44 & 90.80 &  71.59 \\
  Cross-Modal & & TF & 63.10 & 0.4710 & 50.67 & 51.94 & 89.19 & 68.06  \\
 Transformer \cite{pradeepkumar2022towards}& & KD (Offline) & 69.20 & 0.5571 & 56.31 & 56.27 & 95.38 & 71.55 \\   
  & &  KD (Online) & 68.56 & 0.5523 & 56.35 & 57.46 & 90.85 & 72.25 \\
 \hline


%\multirow{2}{*}{\textbf{Dataset}}
% \vspace{-1.3em}
\end{tabular}
\vspace{-2em}
\label{table:results}
% \end{adjustwidth}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



